MOTIF: A tool for Mutation Testing with Fuzzing

Mutation testing consists of generating test cases that detect faults injected into software (generating mutants) which its original test suite could not. By running such an augmented set of test cases, it may discover actual faults that may have gone unnoticed with the original test suite. It is thus a desired practice for embedded software running in safety-critical cyber-physical systems (CPS). Unfortunately, the state-of-the-art tool targeting C, a typical language for CPS software, relies on symbolic execution, whose limitations often prevent its application. MOTIF overcomes such limitations by leveraging grey-box fuzzing tools to generate unit test cases in C that detect injected faults in mutants. Indeed, fuzzing tools automatically generate inputs by exercising the compiled version of the software under test guided by coverage feedback, thus overcoming the limitations of symbolic execution. Our empirical assessment has shown that it detects more faults than symbolic execution (i.e., up to 47 percentage points), when the latter is applicable.

==> listings/asn.tex <==
% !TEX root =  ../MAIN.tex

\begin{minipage}{8cm}
\begin{lstlisting}[style=CStyle, caption=Excerpt of the tested ASN.1 grammar., label=asn_excerpt, mathescape=true]
MyInt ::= INTEGER (0 .. 20)

My2ndInt ::= MyInt ( 1 .. 18)

AType ::= SEQUENCE {
    blArray SEQUENCE (SIZE(10)) OF BOOLEAN
}

My2ndAType ::= AType

TypeNested ::= SEQUENCE {
    intVal  INTEGER(0..10),
    int2Val INTEGER(-10..10),
    int3Val MyInt (10..12),
    intArray    SEQUENCE (SIZE (10)) OF INTEGER (0..3),
    realArray   SEQUENCE (SIZE (10)) OF REAL (0.1 .. 3.14),
    octStrArray SEQUENCE (SIZE (10)) OF OCTET STRING (SIZE(1..10)),
    boolArray   SEQUENCE (SIZE (10)) OF T-BOOL,
    label   OCTET STRING (SIZE(10..40)),
    bAlpha  T-BOOL,
    bBeta   BOOLEAN,
    sString T-STRING,
    arr     T-ARR,
    arr2    T-ARR2
}

E ::= INTEGER (0..255|1299)(5)
\end{lstlisting}
\end{minipage}



==> listings/probeExample.tex <==
%\begin{minipage}[t]{8.4cm}
\begin{lstlisting}[style=CStyle, mathescape=true, caption=Example of \APPR mutation probes (in bold)., label=lst:mutationProbes]
...
switch(message_type)
	case IfStatus:
		GetIfStatus(buffer);
		$\textbf{mutate\_FM\_IfStatus( buffer)}$;
		break;
	case IfHouseKeeping:
		GetIfHouseKeeping(buffer);
		$\textbf{mutate\_FM\_IfHK( buffer )}$;
		break;		
 ...
 \end{lstlisting}
%\end{minipage}

% 		$\textbf{\_unload\_FM(fm)}$;
% $\textbf{\_unload\_FM(fm)}$;

==> listings/selection.tex <==
% !TEX root =  ../MAIN.tex

\newcommand{\INDA}{10}
\newcommand{\INDB}{15}
\newcommand{\INDC}{5}

%\vspace{-3mm}
\begin{figure}[tb]

\begin{algorithmic}[1]

%\footnotesize
\scriptsize

\Require \emph{TS}, the test suite of the software under test
\Require \emph{Cov}, coverage information, for each test case
\Require \emph{ms}, the mutated statement
\Ensure \emph{PTS}, a list of test cases to be executed, sorted by priority
% (source inputs, follow-up inputs, output data).

\State $\mathit{TS}_m \gets$ subset of $\mathit{TS}$ that cover the mutated statement $\mathit{ms}$, based on \emph{Cov} \label{alg:prioritize:select}
\State $\mathit{PTS} \gets \mathit{new} \mathit{list}$ \textcolor{darkgray}{//this list is initially empty}
\State $\mathit{PTS} \gets$ based on \emph{Cov} select from $\mathit{TS_m}$ the test case $t$ that exercises $\mathit{ms}$ more times \label{alg:prioritize:first}
\State $\mathit{PTS} \gets \mathit{PTS} \cup t$ \textcolor{darkgray}{//include first the test case selected above}  \label{alg:prioritize:add}

\State \textbf{repeat} \label{alg:prioritize:repeat}
\State \hspace{\INDC mm} \textbf{for each} $n$ in ($\mathit{TS}_m$ - $\mathit{PTS}$) \textcolor{darkgray}{, i.e., is the set of test cases not already added to $\mathit{PTS}$} \label{alg:prioritize:notSel}
\State \hspace{\INDA mm} \textbf{for each} $t$ in $\mathit{PTS}$
\State \hspace{\INDB mm} compute the distance between $t$ and $n$
\State \hspace{\INDA mm} identify $t_n$ i.e., the test case $t$ with the minimal $d$ \label{alg:prioritize:minD}
\State \hspace{\INDC mm} among all the $t_n$ identified, select the one with the highest distance $d$ \label{alg:prioritize:selectStart}
\State \hspace{\INDC mm} \textbf{if} $d > 0$ \textcolor{darkgray}{//there is at least a test case with a different coverage}
\State \hspace{\INDA mm} \textcolor{darkgray}{//note: $n$ is the test case in the set ($\mathit{TS}_m$ - $\mathit{PTS}$) closer to $t_n$}
\State \hspace{\INDA mm} $\mathit{PTS} \gets \mathit{PTS} \cup n$ \label{alg:prioritize:selectEnd}
\State \textbf{until} $d > 0$ \label{alg:prioritize:until}

\end{algorithmic}
\vspace{-3mm}
\caption{PrioritizeAndReduce: Algorithm for prioritizing test cases}
%\vspace{-0.2cm}
\label{alg:prioritize}
\end{figure}


==> listings/semuDriver.tex <==
% !TEX root =  ../MAIN.tex

%\begin{minipage}{8cm}

% typedef enum {
%     T_POS_NONE,
%     longitude_PRESENT,
%     latitude_PRESENT,
%     height_PRESENT,
%     subTypeArray_PRESENT,
%     label_PRESENT,
%     intArray_PRESENT,
%     myIntSet_PRESENT,
%     myIntSetOf_PRESENT,
%     anInt_PRESENT
% } T_POS_selection;


% typedef struct {
%     T_POS_selection kind;

%     union {
%         asn1Real longitude;
%         asn1Real latitude;
%         asn1Real height;
%         T_POS_subTypeArray subTypeArray;
%         T_POS_label label;
%         T_ARR intArray;
%         T_SET myIntSet;
%         T_SETOF myIntSetOf;
%         My2ndInt anInt;
%     } u;
% } T_POS;

\begin{lstlisting}[style=CStyle, tabsize=2, caption=Example \SEMU driver corresponding to the fuzzing driver in~Listing~\ref{asn_driver}., label=semu_driver, mathescape=true]
int main(int argc, char** argv){
    // Declare variable to hold function returned value
    _Bool result;
    // Declare arguments and make input ones symbolic
    T_POS pVal;
    int pErrCode;
    
    klee_make_symbolic(&pVal, sizeof(pVal), "pVal");
    // Call function under test
    result = T_POS_IsConstraintValid(&pVal, &pErrCode);
    // Print output data
    printf("pErrCode = %d\n", pErrCode);
    printf("result = %d\n", result);
    return (int)result;
}
    
\end{lstlisting}
%\end{minipage}



==> listings/test.tex <==
% !TEX root =  ../MAIN.tex

%\begin{minipage}{8cm}

% typedef enum {
%     T_POS_NONE,
%     longitude_PRESENT,
%     latitude_PRESENT,
%     height_PRESENT,
%     subTypeArray_PRESENT,
%     label_PRESENT,
%     intArray_PRESENT,
%     myIntSet_PRESENT,
%     myIntSetOf_PRESENT,
%     anInt_PRESENT
% } T_POS_selection;


% typedef struct {
%     T_POS_selection kind;

%     union {
%         asn1Real longitude;
%         asn1Real latitude;
%         asn1Real height;
%         T_POS_subTypeArray subTypeArray;
%         T_POS_label label;
%         T_ARR intArray;
%         T_SET myIntSet;
%         T_SETOF myIntSetOf;
%         My2ndInt anInt;
%     } u;
% } T_POS;

\begin{figure}
\caption{Example test case for a function \texttt{T\_POS\_IsConstraintValid}.}
\label{asn_test} 
\begin{lstlisting}[style=CStyle, tabsize=2, mathescape=true]
/*Variables with the data in the file killing the mutant*/
const char input_data_pVal={0xFF,0xFF,...,0xFF};
const char input_data_pErrCode={0xFF,0xFF,0xFF,0xFF};
/*Variables with the values observed after mutation testing*/
const char expected_pVal={0xFF,0xFF,...,0xFF};
const char expected_pErrCode={0xFF,0xFF,0xFF,0xFF};
const char expected_return={0x00,0x00,0x00,0x00};
/*Test case*/
int main(int argc, char** argv){
  T_POS pVal;
  int pErrCode;
  int _return;
  /*Initialize inputs*/
  memcopy(&pVal, input_data_pVal, sizeof(pVal));
  memcopy(&pErrCode, input_data_pErrCode, sizeof(int));
  /* Invoke the original function*/
  _return = T_POS_IsConstraintValid(&pVal, &pErrCode);
  /* Print output values of the original function */
  printf_struct("pVal (T_POS)=", &pVal, sizeof(pVal));
  printf("pErrCode (int) = %d\n", pErrCode);
  printf("return (flag) = %d\n", _return);
  /* Generated assertions enabling  regression testing*/
  assert( 0==compare((char*)&pVal, sizeof(pVal)));
  assert( 0==compare((char*)&pErrCode, sizeof(pErrCode)));
  assert( 0==compare((char*)&_return, sizeof(_return)));
  return 0;
}
\end{lstlisting}
\end{figure}
%\end{minipage}



==> listings/types.tex <==
% \hspace*{-\parindent}%
% \begin{minipage}{\linewidth}
\begin{lstlisting}[
style=CStyle, 
tabsize=2,
% caption=Input types for the mutated function \texttt{T\_POS\_IsConstraintValid}, 
caption=Definition of \texttt{struct T\_POS}, 
label=asn_types, 
mathescape=true
]
typedef enum { T_POS_NONE,           longitude_PRESENT, 
               latitude_PRESENT,     height_PRESENT, 
               subTypeArray_PRESENT, label_PRESENT, 
               intArray_PRESENT,     myIntSet_PRESENT, 
               myIntSetOf_PRESENT,   anInt_PRESENT
} T_POS_selection;

typedef struct {
    T_POS_selection kind;
    union { asn1Real longitude; asn1Real latitude; 
            asn1Real height;    My2ndInt anInt; 
            T_POS_label label;  T_ARR intArray; 
            T_SET myIntSet;     T_SETOF myIntSetOf; 
            T_POS_subTypeArray subTypeArray; 
    } u;
} T_POS;
\end{lstlisting}
% \vspace{-0.5em}
% \end{minipage}

==> sections/related.tex <==
% !TEX root = MAIN.tex

\section{Related Work}
\label{sec:related}




We focus on mutation testing tools targeting C/C++ software.  The SOTA tool is \SEMU~\cite{Chekam2021}, which relies on SE and was described in the Introduction. Other SE approaches are outdated~\cite{holling2016nequivack,riener2011test}.
Some SE limitations are overcome by dynamic SE (DSE), which consists of combining the results of program interpretation with real data; however, only compilation-based approaches like QSYM~\cite{yun2018qsym} and SYMCC~\cite{SymCC} do not need additional modeling of the environment.
Nevertheless, a more effective testing solution is \emph{hybrid fuzzing}, which relies on grey-box fuzzing to explore most of the execution paths of a program and leverages DSE to explore branches that are guarded by narrow-ranged constraints. However, existing hybrid fuzzers rely on either SYMCC or QSYM, which makes them inapplicable to CPS software; indeed, SYMCC relies on LLVM, which is not applicable to certain systems~\cite{Oscar:TSE}, while QSYM relies on an outdated version of the PIN instrumenter~\cite{PIN:paper}.

Other approaches rely on \emph{meta-heuristic search}. Souza et al.~\cite{souza2016strong} extends AUSTIN, a search-based testing tool for C~\cite{LAKHOTIA2013112}, but such extension is not available. 
Another key limitation of AUSTIN is that it implements preprocessing steps that do not work with complex program structures (e.g., we couldn't apply them to our subject programs).
%Also the search-based approach of Dang et al.~\cite{dang2019efficiently} is not available.
Another search-based approach is that of Dang et al.~\cite{dang2019efficiently}, but it is not available as well.

The work of Bingham~\cite{brown2020mutation} is the only one relying on \emph{fuzzing to automate mutation testing for C software}; however, instead of generating unit test cases, it generates input files matching a given grammar.
Further, Bingham's results are preliminary and no prototype tool is available.
The only other work relying on fuzzing for mutation testing is Mu2~\cite{MU2}, which targets Java programs. It relies on the mutation score to drive the generation of test inputs. Different from \MOTIF, Mu2 exercises every live mutant with each generated input and, in the file pool, prioritizes those files that increase the mutation score; scalability is achieved by dynamic classloading and instrumentation, two options that are feasible for Java but not for C/C++ programs. 


==> sections/tool_overview.tex <==
% !TEX root =  MAIN.tex

\section{MASS methodology}
\label{sec:overview}

\begin{figure}[tb]
\includegraphics[width=0.875\columnwidth]{images/Approach}
\caption{Workflow of the \MASS approach. }
\label{fig:methodology}
\end{figure}

\MASS is the tool supporting our methodology for the mutation analysis of embedded software within CPS~\cite{Cornejo:2021:TSE}. 
%In this section, we describe the tool and provide details about the procedures performed in each step of the methodology.
% Figure~\ref{fig:approach} shows the eight steps of the methodology implemented by \MASS.
\MASS performs mutation analysis in eight steps, which are depicted in Figure~\ref{fig:methodology}.

In \emph{Step 1}, \MASS collects the SUT code coverage.
Code coverage enables some optimizations such as not mutating statements that are not covered by the test suite, and executing only the test cases that cover a mutated statement.

% \input{tables/mass_operators}

In \emph{Step 2}, \MASS generates mutants by relying on an extended sufficient set of operators, which consists of ABS, AOR, ICR, LCR, ROR, SDL, UOI, AOD, LOD, ROD, BOD, SOD, and LVR~\cite{Cornejo:2021:TSE}. % which are listed in Table~\ref{table:operators}.

In \emph{Step 3}, \MASS compiles the mutants in an iterative way to leverage the incremental compilation implemented by build systems.
It compiles every mutant within the same source folder structure; for each mutant, it replaces the corresponding original source file with the mutated one and builds the software. The original file is restored after each compilation. This enables the reuse of compiled objects thus saving a considerable amount of time.

%; build systems create one object file for each source file to be compiled and then link these object files together into the final executable. After the first build, in subsequent builds, build systems recompile only the modified files and link them to the rest.
%The idea is to leverage build systems by compiling only the modified files for each mutant (i.e., the mutated file and the file restored to eliminate the previous mutation), this enables the reuse most of the already compiled objects, and thus saving considerable amount of time.

% , after the first build, CPS build systems (e.g., GNU make) will only recompile the source file concerning the mutant being processed, and link the object file into the final executable. This procedure saves considerable amount of time, since it is not necessary the full system for every mutant under analysis.

%Fabrizio: ad citation of GDB
In \emph{Step 4}, \MASS removes equivalent and redundant mutants from the set of generated mutants by relying on compiler optimizations (i.e., O0, O1, O2, O3, O4, Ofast, Os for the GCC compiler~\cite{GDB}). For every optimisation level, \MASS re-compiles every mutant and stores the SHA-512 hash of the generated executable. 
Equivalent and redundant mutants are identified by comparing SHA-512 hashes, which is more efficient than comparing the compiled executables.
%To detect equivalent mutants, \MASS discards all the mutants that possess the same SHA-512 hash with respect to the original program. To detect duplicate mutants, \MASS discards all the mutants that possess the same SHA-512 hash between themselves.
%In mutation analysis, equivalent and duplicate mutants prevent the correct assessment of test suite adequacy, since these mutants produce the same output of the original software (i.e., equivalent mutants) or produce the same output with other mutants but a different output with respect to the original program (i.e., duplicate mutants).

%Fabrizio: add required citations below
To further address scalability issues, in \emph{Step 5}, \MASS samples mutants from the set of compiled, nonequivalent, and nonredundant mutants.
%\emph{Duplicate} mutants are a type of redundant mutants. These mutants are equivalent to each other but not equivalent to the original program. We do not target \emph{subsumed} mutants, (i.e., mutants that are not equivalent with each other but are killed by the same test cases), another type of redundant mutants, since it would require test suites that distinguish every mutant from each other, which is out of the scope of this work.
\MASS supports \emph{proportional uniform sampling}~\cite{zhang2013operator}, \emph{proportional method-based sampling}~\cite{zhang2013operator}, \emph{uniform fixed-size sampling}~\cite{gopinath2015hard}, and \emph{FSCI-based sampling}. \emph{Proportional uniform sampling} randomly samples a user-specified percentage of mutants, \emph{proportional method-based sampling} randomly samples a user-specified percentage of mutants for each method of the SUT,
\emph{uniform fixed-size sampling} randomly samples a user-specified number of mutants across the whole program. 
\emph{FSCI-based sampling} (hereafter, FSCI) determines the sample size dynamically while exercising mutants, based on a fixed-width sequential confidence interval approach~\cite{Frey:FixedWidthSequentialConfidenceIntervals:AmericanStatistician:2010}. %put the reference we had in the background section of TSE
With FSCI, \MASS iteratively selects a random mutant and exercises it with the SUT test suite; the process stops when the confidence interval computed with the Clopper-Pearson method~\cite{ClopperPearson} is below a user-specified threshold (defaults to $0.10$). Since FSCI enables \MASS to provide statistical guarantees about the accuracy of the estimated mutation score (see Section~\ref{sec:evaluation}), we therefore recommend its use. 
%the other sampling methods are provided for experimental purposes.
\emph{FSCI} is a novel feature of \MASS.

%We suggest using \emph{FSCI} because is the strategy that enables the test of the smallest number of mutants while maintaining a high accuracy . Note that, even though 


% \input{listings/selection}

In \emph{Step 6}, \MASS executes a prioritized and reduced set of test cases for each mutant. First, \MASS selects only the test cases that cover the mutated statement. Second, \MASS defines the order of execution of test cases based on the likelihood of killing a mutant. To determine this likelihood, we rely on code coverage to determine how dissimilar two test cases are and compare the number of times each statement has been covered by test cases. To measure the distance between two test cases we use the cosine similarity distance. %The complete algorithm for selecting and prioritizing test cases is described in Figure~\ref{alg:prioritize}.

In \emph{Step 7}, \MASS identifies likely equivalent mutants based on code coverage; a mutant is likely equivalent when the cosine similarity distance from the original program is equal to zero; such threshold has been empirically determined~\cite{Cornejo:2021:TSE}.
 %note that \MASS only consider live mutants for this task. 
Redundant mutants cannot be identified with this method because it has not been possible to empirically determine a threshold for this purpose~\cite{Cornejo:2021:TSE}; such finding is probably due to test suites being typically unable to distinguish redundant mutants~\cite{shin2017theoretical}.

In \emph{Step 8}, \MASS estimates the mutation score as the number of killed mutants divided by the number of total mutants, excluding equivalent and redundant mutants. \MASS also reports other relevant metrics such as statement coverage, the number of executed mutants, and the number of killed and live mutants.

==> tables/actual_ms.tex <==
% !TEX root =  ../MAIN.tex

\begin{table}[tb]
\caption{Actual mutation scores across subjects.}
\label{table:results:accuracy:full} 
\scriptsize
\centering
\begin{tabular}{|
@{\hspace{1pt}}p{7mm}|
@{\hspace{1pt}}>{\raggedleft\arraybackslash}p{10mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{9mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{9mm}@{\hspace{1pt}}|
 >{\raggedleft\arraybackslash}p{19mm}@{\hspace{1pt}}|
}
\hline
\textbf{Subject}&\textbf{Mutants}&\textbf{Killed}&\textbf{Live}&\textbf{Mutation Score (\%)}\\ 
\hline
\emph{ESAIL}$_S$ & 3,536 & 2,311  & 1,225  & 65.36 \\
\LIBCSP&4,982&3,270&1,712&65.64 \\
\LIBPARAM&3,931&2,717&1,214&69.12 \\
\LIBUTIL &14,574 & 10,376 & 4,198 & 71.20 \\
\MLFS&21,375&17,484&3,981&81.80 \\
\hline
\end{tabular}

\end{table}


==> tables/caseStudies.tex <==
% !TEX root =  ../Main.tex

\begin{table}[tb]
\caption{Subject artifacts.}
\label{table:caseStudies} 
\footnotesize
\centering
\begin{tabular}{|
@{\hspace{1pt}}p{9mm}
@{\hspace{2pt}}|
@{\hspace{1pt}}>{\raggedleft\arraybackslash}p{16mm}@{\hspace{1pt}}|
@{\hspace{1pt}}>{\raggedleft\arraybackslash}p{8mm}@{\hspace{1pt}}|
@{\hspace{1pt}}>{\raggedleft\arraybackslash}p{15mm}@{\hspace{1pt}}|
@{\hspace{1pt}}>{\raggedleft\arraybackslash}p{26mm}@{\hspace{1pt}}|
@{\hspace{1pt}}>{\raggedleft\arraybackslash}p{9mm}@{\hspace{1pt}}|
}
\hline
\textbf{Subject}&\textbf{Open-source}&\textbf{LOC}&\textbf{\# Test cases}&\textbf{Statements} \textbf{coverage}&\textbf{MS}\\
\hline
%\SAILCSW{}& 2,235 & System& 384 & 95.36\% & 65.36\%\\
%ESAIL execution time: 8.3 hours
\MLFS{}{}& Yes& 5,402 &  4,042 & 100.00\% & 81.80\%\\
\UTIL{}& No& 10,576 & 201 & 83.20\% & 71.20\%\\
%LIBUTIL execution time: 67 seconds
% \ASNLib{}{}& Yes& 4,338 &  107 & 95.8\%\% &61.53\%\\
\ASNLib{}{}& Yes& 7,260 &  139 & 95.80\% &58.31\% \\
%MLFS execution time: 313 seconds (5.2 minutes)
%\MLFS{}{}$_V$& 5402 & 4042 & 100.00\%\\
\hline
\end{tabular}

\end{table}




% \begin{table}[tb]
% \caption{Subject artifacts.}
% \label{table:caseStudies} 
% \footnotesize
% \centering
% \newcommand{\subjtbmargin}{1pt}
% \newcommand{\subjwidth}{15mm}
% \newcommand{\subjwidthsmall}{12mm}
% \newcolumntype{L}[1]{@{\hspace{\subjtbmargin}}
%                      p{#1}
%                      @{\hspace{\subjtbmargin}}
% }
% \newcolumntype{C}[1]{@{\hspace{\subjtbmargin}}
%                      >{\centering\arraybackslash}p{#1}
%                      @{\hspace{\subjtbmargin}}
% }
% \newcolumntype{R}[1]{@{\hspace{\subjtbmargin}}
%                      >{\raggedleft\arraybackslash}p{#1}
%                      @{\hspace{\subjtbmargin}}
% }
% \begin{tabular}{|C{\subjwidth}|C{\subjwidthsmall}|R{\subjwidthsmall}|R{\subjwidthsmall}|R{\subjwidth}|R{\subjwidthsmall}|
% }
% \hline
%     \multirow{2}{*}{\parbox{\subjwidth}{\centering
%         \textbf{Subject}
%     }} &
%     \multirow{2}{*}{\parbox{\subjwidthsmall}{\centering
%                         \textbf{Open- source}
%     }} &
%     \multirow{2}{*}{\parbox{\subjwidthsmall}{\centering
%         \textbf{LOC}
%     }}&
%     \multirow{2}{*}{\parbox{\subjwidthsmall}{\centering
%         \textbf{\# Test cases}
%     }}&
%     \multirow{2}{*}{\parbox{\subjwidth}{\centering
%         \textbf{Statements coverage}
%     }} &
%     \multirow{2}{*}{\parbox{\subjwidthsmall}{\centering 
%         \textbf{MS}  
%     }}\\
%     & & & & & \\
% \hline
% \MLFS{}{} & Yes & 5,402 &  4,042 & 100.00\% & 81.80\%\\
% \UTIL{}& No& 10,576 & 201 & 83.20\% & 71.20\%\\
% \ASNLib{}{}& Yes& 7,260 &  139 & 95.80\% &58.31\% \\
% \hline
% \end{tabular}
% \end{table}




==> tables/case_studies.tex <==
% !TEX root =  ../MAIN.tex

\begin{table}[t]
\caption{Case study subjects.}
\label{table:caseStudies} 
\scriptsize
\centering
\begin{tabular}{|
@{\hspace{1pt}}p{13mm}
@{\hspace{2pt}}|
@{\hspace{1pt}}>{\raggedleft\arraybackslash}p{8mm}@{\hspace{1pt}}|
@{\hspace{1pt}}>{\raggedleft\arraybackslash}p{18mm}@{\hspace{1pt}}|
@{\hspace{1pt}}>{\raggedleft\arraybackslash}p{13mm}@{\hspace{1pt}}|
@{\hspace{1pt}}>{\raggedleft\arraybackslash}p{22mm}@{\hspace{1pt}}|
p{20mm}|}
\hline
\textbf{Subject}&\textbf{LOC}&\textbf{Test suite type}&\textbf{\# Test cases}&\textbf{Statements} \textbf{coverage}\\
\hline
% \SAILCSW& 74,155 & System& 384 & 90.38\% \\
\emph{ESAIL}$_S$& 2\,235 & System& 384 & 95.36\%\\
%ESAIL execution time: 8.3 hours
\LIBCSP &9\,836 & Integration& 89 & 63.10\%\\
%LIBCSP execution time: 107 seconds
\LIBPARAM& 3\,179 & Integration& 170 & 77.60\%\\
%LIBPARAM execution time: 50 seconds
\LIBUTIL& 10\,576 & Unit& 201 & 83.20\%\\
%LIBUTIL execution time: 67 seconds
\MLFS& 5\,402 & Unit& 4042 & 100.00\%\\
%MLFS execution time: 313 seconds (5.2 minutes)
%\MLFS{}{}$_V$& 5402 & 4042 & 100.00\%\\
\hline
\end{tabular}

\end{table}




==> tables/execution_times.tex <==
% !TEX root =  ../Main.tex

\begin{table}[tb]
\caption{Execution times (hours) of different strategies.}
\label{table:exectimes} 
\scriptsize
\centering
\begin{tabular}{|
>{\raggedleft\arraybackslash}p{10mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{20mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{18mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{18mm}@{\hspace{1pt}}|
}
\hline

&\multicolumn{3}{c|}{\textbf{Execution Strategy}}\\
\cline{2-4}
\textbf{Subject}&\textbf{All mutants + Original test suite}&\textbf{FSCI + Original test suite}&\textbf{FSCI + Test suite reduction}\\ 
\hline

\SAIL{}$_{S}$&11\,001.24&2\,804.06&1\,865.73\\

\LIBCSP{}&70.22&12.97&14.91\\
\LIBPARAM{}&13.32&4.21&3.03\\
\LIBUTIL{}&59.45&9.97&6.34\\
\MLFS{}{}&47.72&13.89&9.00\\
\hline
\end{tabular}

\end{table}

==> tables/experimentsMagnitude.tex <==
% !TEX root =  ../MAIN.tex

\begin{table}[tb]
\caption{Scale of experiments.}
\label{table:magnitude} 
\scriptsize
\centering
\begin{tabular}{|
@{\hspace{1pt}}p{12mm}
@{\hspace{2pt}}|
@{\hspace{1pt}}>{\raggedleft\arraybackslash}p{25mm}@{\hspace{1pt}}|
@{\hspace{1pt}}>{\raggedleft\arraybackslash}p{30mm}@{\hspace{1pt}}|
p{20mm}|}
\hline
\textbf{Subject}&\textbf{Total test cases executed}&\textbf{Total execution time (minutes)}\\
\hline
\emph{ESAIL}$_S$&  302,158 & 1,624,336\\
\LIBCSP&  771,274 & 33,756\\
\LIBPARAM&  1,094,800 & 7,205\\
\LIBUTIL&  4,481,295 & 57,732\\
\MLFS&  170,303,452 & 189,633\\
\hline
\textbf{Total}&  176,952,979 & 1,912,662\\
\hline
\end{tabular}

\end{table}


==> tables/fsci.tex <==
% !TEX root =  ../MAIN.tex

\begin{table*}[h]
\caption{Accuracy with proportional uniform sampling (uniform), uniform fixed-size sampling (fixed) and FSCI sampling.}
\label{table:results:accuracy:FSCI:sampling} 
\scriptsize
\centering
\begin{tabular}{|
>{\raggedleft\arraybackslash}p{9mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
p{12mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{9mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
p{12mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{9mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
p{12mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{9mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
p{12mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{9mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
p{12mm}@{\hspace{1pt}}|
}
\hline
\multicolumn{3}{|c|}{\textbf{\LIBCSP}}      & \multicolumn{3}{c|}{\textbf{\LIBPARAM}}      & \multicolumn{3}{c|}{\textbf{\LIBUTIL}}       & \multicolumn{3}{c|}{\textbf{\MLFS}}          & \multicolumn{3}{c|}{\textbf{\emph{ESAIL}}$_S$}       \\
\hline
\textbf{\#Mutants} & $\delta_{acc}$ & \textbf{Method}   & \textbf{\#Mutants} & $\delta_{acc}$ & \textbf{Method}   & \textbf{\#Mutants} & $\delta_{acc}$ & \textbf{Method}   & \textbf{\#Mutants} & $\delta_{acc}$ & \textbf{Method}   & \textbf{\#Mutants} & $\delta_{acc}$ & \textbf{Method} \\
\hline
50&13.64&uniform 0.01&40&12.19&uniform 0.01&100&7.32&fixed&100&7.80&fixed&36&14.04&uniform 0.01\\
200&5.86&fixed&100&10.17&fixed&146&7.54&uniform 0.01&200&5.20&fixed&100&8.89&fixed\\
250&7.07&uniform 0.05&197&6.98&uniform 0.05&200&5.73&fixed&214&\textbf{4.90}&uniform 0.01&177&6.39&uniform 0.05\\
300&\textbf{4.48}&fixed&200&6.12&fixed&300&5.37&fixed&248&\textbf{4.56}&FSCI&200&6.14&fixed\\
364&\textbf{4.42}&FSCI&300&5.88&fixed&333&\textbf{4.73}&FSCI&300&\textbf{4.04}&fixed&300&5.53&fixed\\
400&5.49&fixed&346&\textbf{4.26}&FSCI&400&\textbf{4.45}&fixed&400&\textbf{3.80}&fixed&354&5.26&uniform 0.1\\
499&\textbf{4.61}&uniform 0.1&394&\textbf{4.36}&uniform 0.1&500&\textbf{3.80}&fixed&500&\textbf{3.11}&fixed&366&\textbf{3.92}&FSCI\\
500&\textbf{3.85}&fixed&400&\textbf{4.27}&fixed&600&\textbf{3.29}&fixed&600&\textbf{2.89}&fixed&400&\textbf{4.52}&fixed\\
600&\textbf{3.65}&fixed&500&\textbf{3.63}&fixed&700&\textbf{3.30}&fixed&700&\textbf{2.80}&fixed&500&\textbf{4.08}&fixed\\
700&\textbf{3.00}&fixed&600&\textbf{3.72}&fixed&729&\textbf{3.11}&uniform 0.05&800&\textbf{2.44}&fixed&600&\textbf{3.73}&fixed\\
800&\textbf{2.90}&fixed&700&\textbf{3.27}&fixed&800&\textbf{3.26}&fixed&900&\textbf{3.02}&fixed&700&\textbf{3.01}&fixed\\
900&\textbf{3.09}&fixed&787&\textbf{3.24}&uniform 0.2&900&\textbf{3.04}&fixed&1000&\textbf{2.35}&fixed&708&\textbf{3.52}&uniform 0.2\\
997&\textbf{2.81}&uniform 0.2&800&\textbf{2.51}&fixed&1000&\textbf{2.31}&fixed&1069&\textbf{2.58}&uniform 0.05&800&\textbf{2.55}&fixed\\
1000&\textbf{2.41}&fixed&900&\textbf{2.50}&fixed&1458&\textbf{2.10}&uniform 0.1&2138&\textbf{1.55}&uniform 0.1&900&\textbf{2.37}&fixed\\
1495&\textbf{2.32}&uniform 0.3&1000&\textbf{2.72}&fixed&2915&\textbf{1.57}&uniform 0.2&4275&\textbf{1.09}&uniform 0.2&1000&\textbf{2.96}&fixed\\
\hline
\end{tabular}

Accurate results (i.e., $\delta_{acc} \le 5\%$) are in bold. \textbf{Legend: }uniform $r$ indicates \emph{proportional uniform sampling} with rate $r$, fixed indicates \emph{uniform fixed-size sampling}, and FSCI indicates \emph{uniform FSCI sampling}.
\end{table*}


==> tables/mass_operators.tex <==
% !TEX root =  ../MAIN.tex

\newcommand{\op}{\mathit{op}}
\newcommand{\ArithmeticSet}{ \texttt{+}, \texttt{-}, \texttt{*}, \texttt{/}, \texttt{\%} }
\newcommand{\LogicalSet}{ \texttt{&&}, \texttt{||} }
\newcommand{\RelationalSet}{ \texttt{>}, \texttt{>=}, \texttt{<}, \texttt{<=}, \texttt{==}, \texttt{!=} }
\newcommand{\BitWiseSet}{ \texttt{\&}, \texttt{|}, \land }
\newcommand{\ShiftSet}{ \texttt{>>}, \texttt{<<} }


\begin{table}[tb]
\caption{Implemented set of mutation operators.}
\label{table:operators} 
\centering
\scriptsize
\begin{tabular}{|@{}p{4mm}@{}|@{}p{1cm}@{\hspace{1pt}}|@{}p{7.1cm}@{}|}
\hline
&\textbf{Operator} & \textbf{Description$^{*}$} \\
\hline
\multirow{7}{*}{\rotatebox{90}{\emph{Sufficient Set}}}&ABS               & $\{(v, -v)\}$	\\
\cline{2-3}
&AOR               & $\{(\op_1, op_2) \,|\, \op_1, \op_2 \in \{ \ArithmeticSet \} \land \op_1 \neq \op_2 \} $       \\
&    			  & $\{(\op_1, \op_2) \,|\, \op_1, \op_2 \in \{\texttt{+=}, \texttt{-=}, \texttt{*=}, \texttt{/=}, \texttt{\%} \texttt{=}\} \land \op_1 \neq \op_2 \} $       \\
\cline{2-3}
&ICR               & $\{i, x) \,|\, x \in \{1, -1, 0, i + 1, i - 1, -i\}\}$           \\
\cline{2-3}
&LCR               & $\{(\op_1, \op_2) \,|\, \op_1, \op_2 \in \{ \texttt{\&\&}, || \} \land \op_1 \neq \op_2 \}$            \\
&				  & $\{(\op_1, \op_2) \,|\, \op_1, \op_2 \in \{ \texttt{\&=}, \texttt{|=}, \texttt{\&=}\} \land \op_1 \neq \op_2 \}$            \\
&				  & $\{(\op_1, \op_2) \,|\, \op_1, \op_2 \in \{ \texttt{\&}, \texttt{|}, \texttt{\&\&}\} \land \op_1 \neq \op_2 \}$            \\
\cline{2-3}
&ROR               & $\{(\op_1, \op_2) \,|\, \op_1, \op_2 \in \{ \RelationalSet \}\}$            \\
&				  & $\{ (e, !(e)) \,|\, e \in \{\texttt{if(e)}, \texttt{while(e)}\} \}$ \\
\cline{2-3}
&SDL               & $\{(s, \texttt{remove}(s))\}$            \\
\cline{2-3}
&UOI               & $\{ (v, \texttt{--}v), (v, v\texttt{--}), (v, \texttt{++}v), (v, v\texttt{++}) \}$            \\   
\hline
\hline
\multirow{5}{*}{\rotatebox{90}{\emph{OODL}}}&AOD               & $\{((t_1\,op\,t_2), t_1), ((t_1\,op\,t_2), t_2) \,|\, op \in \{ \ArithmeticSet \} \}$       \\ 
\cline{2-3}
&LOD               & $\{((t_1\,op\,t_2), t_1), ((t_1\,op\,t_2), t_2) \,|\, op \in \{ \texttt{\&\&}, || \} \}$       \\ 
\cline{2-3}
&ROD               & $\{((t_1\,op\,t_2), t_1), ((t_1\,op\,t_2), t_2) \,|\, op \in \{ \RelationalSet \} \}$       \\ 
\cline{2-3}
&BOD               & $\{((t_1\,op\,t_2), t_1), ((t_1\,op\,t_2), t_2) \,|\, op \in \{ \BitWiseSet \} \}$       \\ 
\cline{2-3}
&SOD               & $\{((t_1\,op\,t_2), t_1), ((t_1\,op\,t_2), t_2) \,|\, op \in \{ \ShiftSet \} \}$       \\ 
%\hline
%COR               & $\{(\op_1, \op_2) \,|\, \op_1, \op_2 \in \{ \texttt{\&\&}, \texttt{||}, \land \} \land \op_1 \neq \op_2 \}$            \\
\hline
\hline
\multirow{2}{*}{\rotatebox{90}{\emph{Other}}}&LVR			& $\{(l_1, l_2) \,|\, (l_1, l_2) \in \{(0,-1), (l_1,-l_1), (l_1, 0), $\\
&&\hspace{5mm}$(\mathit{true}, \mathit{false}), (\mathit{false}, \mathit{true})\}\}$           \\
\hline
\end{tabular}

$^{*}$Each pair in parenthesis shows how a program element is modified by the mutation operator on the left; we follow standard syntax~\cite{Kintis2018}. Program elements are literals ($l$), integer literals ($i$), boolean expressions ($e$), operators ($\op$), statements ($s$), variables ($v$), and terms ( $t_i$, which might be either variables or literals).
\end{table}


==> tables/mut_tools.tex <==
% !TEX root =  ../MAIN.tex

\begin{table}[ht]

\scriptsize
\centering
\caption{Mutation analysis tools in the literature.}
\begin{center}
\label{table:tools}
\begin{tabular}{|p{3mm}|p{25mm}|p{43mm}|}
\hline
\textbf{Ref.} & \textbf{Tool} & \textbf{Available} \\
\hline
\cite{rothermel1996experimental} & ADA mutation tool & NA\\
\cite{delamaro2001interface} &	Proteum & \url{https://github.com/magsilva/proteum} \\
\cite{chan2005fault} & SQL mutation tool (Chan) & NA \\
\cite{ma2006mujava} & MuJava & \url{https://cs.gmu.edu/~offutt/mujava/}\\
\cite{tuya2007mutating} & SQL mutation tool (Tuya) & NA\\
\cite{jia2008milu} & Milu & \url{https://github.com/yuejia/Milu/} \\
\cite{shahriar2008music} & SQL MUSIC & NA \\
\cite{shahriar2008mutation} & Function calls mutation tool & NA \\
\cite{madeyski2010judy} & Judy & NA \\
\cite{derezinska2011object} & ILMutator & NA \\
\cite{binh2012mutation}	& Simulink mutation tool & NA\\
\cite{mateo2012validating} & Bacterio & NA \\
\cite{dan2012semantic}	& Floating Point mutation tool & NA \\
\cite{just2014major}	& Major & \url{http://mutation-testing.org/} \\
\cite{grechanik2016mutation}	& jMINT & \url{https://github.com/Toparvion/jmint} \\
\cite{delgado2017assessment}	& MuCPP & \url{https://ucase.uca.es/mucpp/} \\
\cite{wang2017faster} & Accmut & \url{https://github.com/wangbo15/accmut}\\
\cite{hariri2018srciror} & SRCiror & \url{https://github.com/TestingResearchIllinois/srciror} \\
\cite{phan2018music} & MUSIC & \url{https://github.com/swtv-kaist/MUSIC} \\
\cite{denisov2018mull}	&  Mull & \url{https://github.com/mull-project/mull} \\
\cite{chekam2020muteria} & Muteria & \url{https://github.com/thierry-tct/muteria}\\
\hline
\end{tabular}
\end{center}
\end{table}%

==> tables/results_ms.tex <==
% !TEX root =  ../Main.tex

\begin{table}[htb]
\caption{\APPR Mutation Score.}
\label{table:results:mutationScore} 
\scriptsize
\centering
\begin{tabular}{|
>{\raggedleft\arraybackslash}p{14mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{26mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{15mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{15mm}@{\hspace{1pt}}|
}
\hline
\textbf{Subject}&\textbf{Predicted Equivalent}&\multicolumn{2}{c|}{\textbf{Mutation Score (\%)}}\\
&\textbf{Mutants Removed (\%)}&\textbf{Traditional}&\textbf{\APPR}\\ 
\hline
% 1225-32=1193; 2311/(2311+1193)
\SAIL{}$_{S}$&2.61&65.36&65.95\\
%$\mathit{\SAIL{}}$&&\\
% 4198-2281=1917; 10376/(10376+1917)


% 1214-770=444; 2717/(2717+444)

% 1712-371=1341; 3270/(3270+1341)
\LIBCSP{}&21.67&65.64&70.92\\
\LIBPARAM{}&63.43&69.12&85.95\\
% 3981-2699=1282; 17484/(17484+1282)
\LIBUTIL{}&54.34&71.20&84.41\\
\MLFS{}{}&69.37&81.80&93.49\\
\hline
$\textbf{Average}$&42.28&70.62&81.14\\
\hline
\end{tabular}

\end{table}

%2021-06-14
%Average MS with reduced test suite, above is with the whole TS
% 
%CSP 70.92
%LIBUTIL 84.41
%PARAM 85.95
%MLFS 93.49
%ESAIL 65.95


==> tables/seeds.tex <==
\begin{table}[t]
\centering
\scriptsize
\caption{Seeds assigned to types}
\label{tab:seedValues}
\begin{tabular}{
|@{\hspace{1pt}}>{\raggedleft\arraybackslash}p{10mm}@{\hspace{1pt}}|
@{\hspace{1pt}}>{\raggedleft\arraybackslash}p{27mm}@{\hspace{1pt}}|
@{\hspace{1pt}}>{\raggedleft\arraybackslash}p{20mm}@{\hspace{1pt}}|
@{\hspace{1pt}}>{\raggedleft\arraybackslash}p{27mm}@{\hspace{1pt}}|}
 \hline
 \textbf{Type}& \textbf{Seed 1}&\textbf{Seed 2}&\textbf{Seed 3}\\
 \hline
int& -1& 0& 1\\
Bool& False& True& \\
float& -3230283776.0& 0.0& 1072693248.0\\ double& 13826050856027422720.0& 0.0&
4602891378046628864.0\\
char& 0xFF& 0x00& 0x41\\
byte& 0xFF& 0x00& 0x41\\
ISO8601& 2145916800.999999999&
1970-01-01T00:00:00Z& 2038-01-01T00:00:00Z\\ 
\hline
\end{tabular}%

%*C means data collected from Crawler and CM means data collected from crawler plus the manual data

\end{table}



% \begin{table}[b]
% \centering
% \scriptsize
% \caption{Seeds assigned to types}
% \label{tab:seedValues}
% \newcommand{\seedcolsize}{16mm}
% \newcommand{\parlinespace}{0.85}
% \newcolumntype{Y}{>{\raggedleft\arraybackslash}p{\seedcolsize}}

% \begin{tabular}{|c|Y|Y|Y|}
% \hline
%     \multicolumn{1}{|c|}{ \textbf{Type} } & 
%     \multicolumn{1}{c|}{ \textbf{Seed 1} } &
%     \multicolumn{1}{c|}{ \textbf{Seed 2} } &
%     \multicolumn{1}{c|}{ \textbf{Seed 3} } \\
% \hline
%     int     & -1      & 0 & 1\\
%     Bool    & False   & True &  True\\
%     float   & -3230283776.0& 0.0& 1072693248.0\\ 
%     \multirow{2}{*}{double}
%             & \multirow{2}{*}{\parbox{\seedcolsize}{
%                 \raggedleft\setstretch{\parlinespace} 138260508560 27422720.0}
%             }
%             & \multirow{2}{*}{0.0}
%             & \multirow{2}{*}{\parbox{\seedcolsize}{
%                 \raggedleft\setstretch{\parlinespace} 46028913780 46628864.0}
%             } \\ 
%             &  & &  \\
%     char    & 0xFF& 0x00& 0x41\\
%     byte    & 0xFF& 0x00& 0x41\\
%     \multirow{2}{*}{ISO8601}
%             & \multirow{2}{*}{\parbox{\seedcolsize}{
%                 \raggedleft\setstretch{\parlinespace} 2145916800. 999999999}
%             }
%             & \multirow{2}{*}{\parbox{\seedcolsize}{
%                 \raggedleft\setstretch{\parlinespace} 1970-01-01T 00:00:00Z}
%                 }
%             & \multirow{2}{*}{\parbox{\seedcolsize}{
%                 \raggedleft\setstretch{\parlinespace} 2038-01-01T 00:00:00Z}
%             }\\ 
%             &  &  & \\
% \hline
% \end{tabular}%
% \end{table}

==> tables/tce.tex <==
% !TEX root =  ../MAIN.tex

\begin{table}[tb]
\caption{Compiler Optimizations Results.}
\label{table:tce} 
\scriptsize
\centering
\begin{tabular}{|
@{\hspace{1pt}}p{8mm}
@{\hspace{2pt}}|
@{\hspace{1pt}}>{\raggedleft\arraybackslash}p{12mm}@{\hspace{1pt}}|
@{\hspace{1pt}}>{\raggedleft\arraybackslash}p{10mm}@{\hspace{1pt}}|
@{\hspace{1pt}}>{\raggedleft\arraybackslash}p{9mm}@{\hspace{1pt}}|
@{\hspace{1pt}}>{\raggedleft\arraybackslash}p{23mm}@{\hspace{1pt}}|
p{9mm}|}
\hline
\textbf{Subject}&\textbf{\# generated mutants}&\textbf{\# mutants compiled}&\textbf{MCT (sec)}&\textbf{\# equivalent and redundant mutants (\%)}&\textbf{\# unique mutants} \\
\hline
\emph{ESAIL}$_S$&7\,212&5\,347&7\,640&1\,811 (33.87)&3\,536\\
\LIBCSP         &8\,666&7\,878&11\,425&2\,896 (36.76)&4\,982\\
\LIBPARAM       &7\,252&6\,440&9\,392&2\,509 (38.96)&3\,931\\
\LIBUTIL        &22\,295&20\,268&30\,624&5\,694 (28.09)&14\,574\\
\MLFS           &31\,526&28\,069&3\,157&6\,694 (23.84)&21\,375\\
\hline
\end{tabular}

\textbf{Legend:} MCT = mutants compilation time.
\end{table}

==> tables/timetable.tex <==
% !TEX root =  ../Main.tex


\begin{table}[tb]
\caption{Statistics of the killed mutants (percentage) over minutes}
\label{table:timetable} 
\footnotesize
\centering
\begin{tabular}{c|rrr|rrr}
\hline
\textbf{Time}  & \multicolumn{3}{c|}{\textbf{MLFS}} & \multicolumn{3}{c}{\textbf{LIBU}} \\
(minute) 
& \multicolumn{1}{c}{min} & \multicolumn{1}{c}{max} & \multicolumn{1}{c|}{avg.}
& \multicolumn{1}{c}{min} & \multicolumn{1}{c}{max} & \multicolumn{1}{c}{avg.} \\
\hline
0 & 1.95\% & 1.95\% & 1.95\% & 49.59\% & 49.75\% & 49.65\% \\
1 & 22.28\% & 23.00\% & 22.69\% & 65.24\% & 66.56\% & 66.13\% \\
2 & 24.34\% & 24.65\% & 24.51\% & 66.06\% & 67.55\% & 66.87\% \\
3 & 25.55\% & 26.14\% & 25.85\% & 66.06\% & 67.55\% & 67.03\% \\
4 & 26.45\% & 26.91\% & 26.67\% & 66.56\% & 67.55\% & 67.13\% \\
5 & 27.24\% & 27.78\% & 27.45\% & 66.56\% & 67.87\% & 67.23\% \\
6 & 27.73\% & 28.27\% & 27.98\% & 66.56\% & 67.87\% & 67.36\% \\
7 & 28.06\% & 28.66\% & 28.39\% & 66.56\% & 68.04\% & 67.64\% \\
8 & 28.40\% & 29.14\% & 28.76\% & 66.72\% & 68.20\% & 67.78\% \\
9 & 28.73\% & 29.50\% & 29.07\% & 67.05\% & 68.37\% & 67.92\% \\
10 & 29.09\% & 29.76\% & 29.38\% & 67.05\% & 68.53\% & 68.02\% \\
11 & 29.30\% & 30.10\% & 29.64\% & 67.05\% & 68.70\% & 68.09\% \\
12 & 29.61\% & 30.25\% & 29.88\% & 67.22\% & 68.70\% & 68.11\% \\
13 & 29.79\% & 30.43\% & 30.09\% & 67.22\% & 68.70\% & 68.12\% \\
14 & 30.07\% & 30.53\% & 30.30\% & 67.22\% & 68.70\% & 68.12\% \\
15 & 30.25\% & 30.71\% & 30.48\% & 67.22\% & 68.70\% & 68.14\% \\
16 & 30.43\% & 30.92\% & 30.65\% & 67.22\% & 68.70\% & 68.14\% \\
17 & 30.56\% & 31.05\% & 30.80\% & 67.22\% & 68.70\% & 68.17\% \\
18 & 30.74\% & 31.25\% & 30.94\% & 67.22\% & 68.70\% & 68.17\% \\
19 & 30.81\% & 31.38\% & 31.05\% & 67.22\% & 68.70\% & 68.17\% \\
20 & 30.89\% & 31.56\% & 31.17\% & 67.22\% & 68.70\% & 68.17\% \\
21 & 30.99\% & 31.74\% & 31.31\% & 67.22\% & 68.70\% & 68.17\% \\
22 & 31.07\% & 31.84\% & 31.43\% & 67.22\% & 68.70\% & 68.20\% \\
23 & 31.17\% & 31.95\% & 31.53\% & 67.22\% & 68.70\% & 68.22\% \\
24 & 31.25\% & 32.02\% & 31.62\% & 67.38\% & 68.70\% & 68.24\% \\
25 & 31.33\% & 32.07\% & 31.72\% & 67.38\% & 68.70\% & 68.24\% \\
26 & 31.46\% & 32.18\% & 31.80\% & 67.38\% & 68.70\% & 68.24\% \\
27 & 31.56\% & 32.20\% & 31.87\% & 67.38\% & 68.70\% & 68.24\% \\
28 & 31.66\% & 32.33\% & 31.97\% & 67.38\% & 68.70\% & 68.24\% \\
29 & 31.71\% & 32.33\% & 32.06\% & 67.38\% & 68.70\% & 68.24\% \\
30 & 31.74\% & 32.38\% & 32.12\% & 67.38\% & 68.70\% & 68.24\% \\
31 & 31.84\% & 32.51\% & 32.20\% & 67.38\% & 68.70\% & 68.24\% \\
32 & 31.97\% & 32.59\% & 32.27\% & 67.38\% & 68.70\% & 68.24\% \\
33 & 32.07\% & 32.64\% & 32.33\% & 67.38\% & 68.70\% & 68.24\% \\
34 & 32.18\% & 32.72\% & 32.39\% & 67.38\% & 68.70\% & 68.24\% \\
35 & 32.25\% & 32.77\% & 32.47\% & 67.38\% & 68.70\% & 68.24\% \\
36 & 32.28\% & 32.82\% & 32.55\% & 67.38\% & 68.70\% & 68.24\% \\
37 & 32.28\% & 32.87\% & 32.61\% & 67.38\% & 68.70\% & 68.24\% \\
38 & 32.38\% & 32.95\% & 32.67\% & 67.38\% & 68.70\% & 68.25\% \\
39 & 32.56\% & 32.97\% & 32.73\% & 67.38\% & 68.70\% & 68.25\% \\
40 & 32.59\% & 33.02\% & 32.79\% & 67.38\% & 68.70\% & 68.27\% \\
41 & 32.67\% & 33.05\% & 32.86\% & 67.38\% & 68.70\% & 68.27\% \\
42 & 32.74\% & 33.13\% & 32.93\% & 67.38\% & 68.70\% & 68.27\% \\
43 & 32.77\% & 33.20\% & 32.99\% & 67.38\% & 68.70\% & 68.27\% \\
44 & 32.82\% & 33.23\% & 33.03\% & 67.38\% & 68.70\% & 68.27\% \\
45 & 32.87\% & 33.33\% & 33.08\% & 67.38\% & 68.70\% & 68.27\% \\
46 & 33.00\% & 33.36\% & 33.13\% & 67.38\% & 68.70\% & 68.27\% \\
47 & 33.02\% & 33.38\% & 33.18\% & 67.38\% & 68.70\% & 68.29\% \\
48 & 33.05\% & 33.46\% & 33.23\% & 67.38\% & 68.70\% & 68.29\% \\
49 & 33.08\% & 33.49\% & 33.27\% & 67.38\% & 68.70\% & 68.29\% \\
50 & 33.18\% & 33.49\% & 33.32\% & 67.38\% & 68.70\% & 68.29\% \\
51 & 33.23\% & 33.54\% & 33.36\% & 67.38\% & 68.70\% & 68.29\% \\
52 & 33.26\% & 33.62\% & 33.40\% & 67.38\% & 68.70\% & 68.29\% \\
53 & 33.26\% & 33.64\% & 33.43\% & 67.38\% & 68.70\% & 68.29\% \\
54 & 33.28\% & 33.74\% & 33.48\% & 67.38\% & 68.70\% & 68.29\% \\
55 & 33.28\% & 33.82\% & 33.52\% & 67.38\% & 68.70\% & 68.29\% \\
56 & 33.28\% & 33.87\% & 33.56\% & 67.38\% & 68.70\% & 68.30\% \\
57 & 33.31\% & 33.92\% & 33.61\% & 67.38\% & 68.70\% & 68.30\% \\
58 & 33.44\% & 33.98\% & 33.67\% & 67.38\% & 68.70\% & 68.30\% \\
59 & 33.44\% & 34.05\% & 33.71\% & 67.38\% & 68.70\% & 68.30\% \\
60 & 33.46\% & 34.05\% & 33.74\% & 67.38\% & 68.70\% & 68.30\% \\
61 & 33.49\% & 34.13\% & 33.78\% & 67.38\% & 68.70\% & 68.30\% \\
62 & 33.49\% & 34.13\% & 33.80\% & 67.38\% & 68.70\% & 68.30\% \\
63 & 33.49\% & 34.16\% & 33.83\% & 67.38\% & 68.70\% & 68.30\% \\
64 & 33.51\% & 34.16\% & 33.88\% & 67.38\% & 68.70\% & 68.30\% \\
65 & 33.54\% & 34.18\% & 33.91\% & 67.38\% & 68.70\% & 68.30\% \\
66 & 33.54\% & 34.21\% & 33.94\% & 67.38\% & 68.70\% & 68.30\% \\
67 & 33.59\% & 34.23\% & 33.97\% & 67.38\% & 68.70\% & 68.30\% \\
68 & 33.64\% & 34.28\% & 34.00\% & 67.38\% & 68.70\% & 68.30\% \\
69 & 33.69\% & 34.28\% & 34.03\% & 67.38\% & 68.70\% & 68.30\% \\
70 & 33.77\% & 34.31\% & 34.07\% & 67.38\% & 68.70\% & 68.30\% \\
\hline
\end{tabular}
\end{table}


\begin{table}[tb]
\caption{Statistics of the killed mutants (percentage) over minutes 2}
\label{table:timetable2} 
\footnotesize
\centering
\begin{tabular}{c|rrr|rrr}
\hline
\textbf{Time}  & \multicolumn{3}{c|}{\textbf{MLFS}} & \multicolumn{3}{c}{\textbf{LIBU}} \\
(minute) 
& \multicolumn{1}{c}{min} & \multicolumn{1}{c}{max} & \multicolumn{1}{c|}{avg.}
& \multicolumn{1}{c}{min} & \multicolumn{1}{c}{max} & \multicolumn{1}{c}{avg.} \\
\hline
71 & 33.82\% & 34.34\% & 34.11\% & 67.38\% & 68.70\% & 68.30\% \\
72 & 33.82\% & 34.41\% & 34.15\% & 67.38\% & 68.70\% & 68.30\% \\
73 & 33.85\% & 34.49\% & 34.19\% & 67.38\% & 68.70\% & 68.30\% \\
74 & 33.87\% & 34.52\% & 34.23\% & 67.38\% & 68.70\% & 68.30\% \\
75 & 33.90\% & 34.57\% & 34.27\% & 67.38\% & 68.70\% & 68.30\% \\
76 & 33.95\% & 34.59\% & 34.30\% & 67.38\% & 68.70\% & 68.30\% \\
77 & 33.98\% & 34.62\% & 34.33\% & 67.38\% & 68.70\% & 68.30\% \\
78 & 34.00\% & 34.64\% & 34.36\% & 67.38\% & 68.70\% & 68.30\% \\
79 & 34.05\% & 34.67\% & 34.39\% & 67.38\% & 68.70\% & 68.30\% \\
80 & 34.05\% & 34.67\% & 34.41\% & 67.38\% & 68.70\% & 68.30\% \\
81 & 34.13\% & 34.72\% & 34.44\% & 67.38\% & 68.70\% & 68.30\% \\
82 & 34.18\% & 34.75\% & 34.47\% & 67.38\% & 68.70\% & 68.30\% \\
83 & 34.21\% & 34.77\% & 34.49\% & 67.38\% & 68.70\% & 68.30\% \\
84 & 34.26\% & 34.77\% & 34.51\% & 67.38\% & 68.70\% & 68.30\% \\
85 & 34.28\% & 34.77\% & 34.53\% & 67.38\% & 68.70\% & 68.30\% \\
86 & 34.31\% & 34.80\% & 34.55\% & 67.38\% & 68.70\% & 68.30\% \\
87 & 34.34\% & 34.82\% & 34.58\% & 67.38\% & 68.70\% & 68.30\% \\
88 & 34.41\% & 34.82\% & 34.61\% & 67.38\% & 68.70\% & 68.30\% \\
89 & 34.44\% & 34.85\% & 34.66\% & 67.38\% & 68.86\% & 68.34\% \\
90 & 34.44\% & 34.85\% & 34.67\% & 67.38\% & 68.86\% & 68.34\% \\
91 & 34.46\% & 34.88\% & 34.70\% & 67.38\% & 68.86\% & 68.34\% \\
92 & 34.46\% & 34.90\% & 34.71\% & 67.38\% & 68.86\% & 68.34\% \\
93 & 34.46\% & 34.93\% & 34.73\% & 67.38\% & 68.86\% & 68.34\% \\
94 & 34.49\% & 34.93\% & 34.74\% & 67.38\% & 68.86\% & 68.34\% \\
95 & 34.49\% & 35.00\% & 34.76\% & 67.38\% & 68.86\% & 68.34\% \\
96 & 34.57\% & 35.00\% & 34.78\% & 67.38\% & 68.86\% & 68.34\% \\
97 & 34.62\% & 35.00\% & 34.81\% & 67.38\% & 68.86\% & 68.34\% \\
98 & 34.64\% & 35.03\% & 34.83\% & 67.38\% & 68.86\% & 68.34\% \\
99 & 34.64\% & 35.06\% & 34.84\% & 67.38\% & 68.86\% & 68.34\% \\
100 & 34.64\% & 35.06\% & 34.86\% & 67.38\% & 68.86\% & 68.34\% \\
101 & 34.67\% & 35.06\% & 34.87\% & 67.38\% & 68.86\% & 68.34\% \\
102 & 34.67\% & 35.06\% & 34.89\% & 67.38\% & 68.86\% & 68.34\% \\
103 & 34.67\% & 35.06\% & 34.90\% & 67.38\% & 68.86\% & 68.34\% \\
104 & 34.72\% & 35.06\% & 34.92\% & 67.38\% & 68.86\% & 68.34\% \\
105 & 34.77\% & 35.08\% & 34.93\% & 67.38\% & 68.86\% & 68.34\% \\
106 & 34.77\% & 35.13\% & 34.96\% & 67.38\% & 68.86\% & 68.34\% \\
107 & 34.77\% & 35.16\% & 34.98\% & 67.38\% & 68.86\% & 68.34\% \\
108 & 34.77\% & 35.18\% & 35.00\% & 67.38\% & 68.86\% & 68.34\% \\
109 & 34.80\% & 35.18\% & 35.02\% & 67.38\% & 68.86\% & 68.34\% \\
110 & 34.80\% & 35.21\% & 35.03\% & 67.38\% & 68.86\% & 68.34\% \\
111 & 34.82\% & 35.21\% & 35.05\% & 67.38\% & 68.86\% & 68.34\% \\
112 & 34.82\% & 35.21\% & 35.06\% & 67.38\% & 68.86\% & 68.34\% \\
113 & 34.93\% & 35.24\% & 35.08\% & 67.38\% & 68.86\% & 68.34\% \\
114 & 34.98\% & 35.24\% & 35.10\% & 67.38\% & 68.86\% & 68.34\% \\
115 & 35.00\% & 35.26\% & 35.11\% & 67.38\% & 68.86\% & 68.34\% \\
116 & 35.00\% & 35.31\% & 35.13\% & 67.38\% & 68.86\% & 68.34\% \\
117 & 35.00\% & 35.31\% & 35.13\% & 67.38\% & 68.86\% & 68.34\% \\
118 & 35.03\% & 35.31\% & 35.15\% & 67.38\% & 68.86\% & 68.34\% \\
119 & 35.06\% & 35.31\% & 35.18\% & 67.38\% & 68.86\% & 68.34\% \\
120 & 35.06\% & 35.31\% & 35.18\% & 67.38\% & 68.86\% & 68.34\% \\
121 & 35.06\% & 35.31\% & 35.20\% & 67.38\% & 68.86\% & 68.35\% \\
122 & 35.06\% & 35.34\% & 35.22\% & 67.38\% & 68.86\% & 68.37\% \\
123 & 35.11\% & 35.36\% & 35.25\% & 67.38\% & 68.86\% & 68.37\% \\
124 & 35.13\% & 35.39\% & 35.26\% & 67.38\% & 68.86\% & 68.37\% \\
125 & 35.13\% & 35.39\% & 35.28\% & 67.38\% & 68.86\% & 68.37\% \\
126 & 35.13\% & 35.39\% & 35.28\% & 67.38\% & 68.86\% & 68.37\% \\
127 & 35.13\% & 35.47\% & 35.30\% & 67.38\% & 68.86\% & 68.37\% \\
128 & 35.18\% & 35.49\% & 35.32\% & 67.38\% & 68.86\% & 68.37\% \\
129 & 35.18\% & 35.52\% & 35.34\% & 67.38\% & 68.86\% & 68.37\% \\
130 & 35.18\% & 35.52\% & 35.35\% & 67.38\% & 68.86\% & 68.37\% \\
131 & 35.18\% & 35.52\% & 35.36\% & 67.38\% & 68.86\% & 68.37\% \\
132 & 35.18\% & 35.54\% & 35.37\% & 67.38\% & 68.86\% & 68.37\% \\
133 & 35.21\% & 35.54\% & 35.38\% & 67.38\% & 68.86\% & 68.37\% \\
134 & 35.24\% & 35.54\% & 35.39\% & 67.38\% & 68.86\% & 68.37\% \\
135 & 35.24\% & 35.54\% & 35.40\% & 67.38\% & 68.86\% & 68.37\% \\
136 & 35.24\% & 35.57\% & 35.42\% & 67.38\% & 68.86\% & 68.37\% \\
137 & 35.24\% & 35.57\% & 35.43\% & 67.38\% & 68.86\% & 68.37\% \\
138 & 35.24\% & 35.65\% & 35.45\% & 67.38\% & 68.86\% & 68.37\% \\
139 & 35.24\% & 35.67\% & 35.46\% & 67.38\% & 68.86\% & 68.37\% \\
140 & 35.26\% & 35.67\% & 35.47\% & 67.38\% & 68.86\% & 68.39\% \\
\hline
\end{tabular}
\end{table}


\begin{table}[tb]
\caption{Statistics of the killed mutants (percentage) over minutes 3}
\label{table:timetable3} 
\footnotesize
\centering
\begin{tabular}{c|rrr|rrr}
\hline
\textbf{Time}  & \multicolumn{3}{c|}{\textbf{MLFS}} & \multicolumn{3}{c}{\textbf{LIBU}} \\
(minute) 
& \multicolumn{1}{c}{min} & \multicolumn{1}{c}{max} & \multicolumn{1}{c|}{avg.}
& \multicolumn{1}{c}{min} & \multicolumn{1}{c}{max} & \multicolumn{1}{c}{avg.} \\
\hline
141 & 35.31\% & 35.70\% & 35.50\% & 67.38\% & 68.86\% & 68.39\% \\
142 & 35.31\% & 35.70\% & 35.50\% & 67.38\% & 68.86\% & 68.39\% \\
143 & 35.34\% & 35.70\% & 35.52\% & 67.38\% & 68.86\% & 68.39\% \\
144 & 35.34\% & 35.70\% & 35.53\% & 67.38\% & 68.86\% & 68.39\% \\
145 & 35.36\% & 35.72\% & 35.55\% & 67.38\% & 68.86\% & 68.39\% \\
146 & 35.36\% & 35.72\% & 35.55\% & 67.38\% & 68.86\% & 68.39\% \\
147 & 35.36\% & 35.72\% & 35.55\% & 67.38\% & 68.86\% & 68.39\% \\
148 & 35.39\% & 35.72\% & 35.57\% & 67.38\% & 68.86\% & 68.39\% \\
149 & 35.39\% & 35.75\% & 35.59\% & 67.38\% & 68.86\% & 68.39\% \\
150 & 35.39\% & 35.75\% & 35.59\% & 67.38\% & 68.86\% & 68.39\% \\
151 & 35.44\% & 35.77\% & 35.62\% & 67.38\% & 68.86\% & 68.39\% \\
152 & 35.44\% & 35.77\% & 35.63\% & 67.38\% & 68.86\% & 68.39\% \\
153 & 35.47\% & 35.80\% & 35.64\% & 67.38\% & 68.86\% & 68.39\% \\
154 & 35.47\% & 35.80\% & 35.64\% & 67.38\% & 68.86\% & 68.39\% \\
155 & 35.47\% & 35.83\% & 35.65\% & 67.38\% & 68.86\% & 68.39\% \\
156 & 35.47\% & 35.85\% & 35.67\% & 67.38\% & 68.86\% & 68.39\% \\
157 & 35.47\% & 35.85\% & 35.67\% & 67.38\% & 68.86\% & 68.39\% \\
158 & 35.49\% & 35.88\% & 35.69\% & 67.38\% & 68.86\% & 68.39\% \\
159 & 35.49\% & 35.88\% & 35.70\% & 67.38\% & 68.86\% & 68.39\% \\
160 & 35.49\% & 35.93\% & 35.72\% & 67.38\% & 68.86\% & 68.39\% \\
161 & 35.52\% & 36.01\% & 35.74\% & 67.38\% & 68.86\% & 68.39\% \\
162 & 35.54\% & 36.01\% & 35.76\% & 67.38\% & 68.86\% & 68.39\% \\
163 & 35.59\% & 36.03\% & 35.79\% & 67.38\% & 68.86\% & 68.39\% \\
164 & 35.59\% & 36.06\% & 35.81\% & 67.38\% & 68.86\% & 68.39\% \\
165 & 35.59\% & 36.06\% & 35.82\% & 67.38\% & 68.86\% & 68.39\% \\
166 & 35.59\% & 36.08\% & 35.83\% & 67.38\% & 68.86\% & 68.39\% \\
167 & 35.59\% & 36.11\% & 35.85\% & 67.38\% & 68.86\% & 68.39\% \\
168 & 35.59\% & 36.11\% & 35.85\% & 67.38\% & 68.86\% & 68.39\% \\
169 & 35.59\% & 36.11\% & 35.85\% & 67.38\% & 68.86\% & 68.39\% \\
170 & 35.59\% & 36.11\% & 35.85\% & 67.38\% & 68.86\% & 68.39\% \\
171 & 35.59\% & 36.11\% & 35.85\% & 67.38\% & 68.86\% & 68.39\% \\
172 & 35.59\% & 36.11\% & 35.85\% & 67.38\% & 68.86\% & 68.39\% \\
173 & 35.59\% & 36.11\% & 35.85\% & 67.38\% & 68.86\% & 68.39\% \\
174 & 35.59\% & 36.11\% & 35.85\% & 67.38\% & 68.86\% & 68.39\% \\
175 & 35.59\% & 36.11\% & 35.85\% & 67.38\% & 68.86\% & 68.39\% \\
176 & 35.59\% & 36.11\% & 35.85\% & 67.38\% & 68.86\% & 68.39\% \\
177 & 35.59\% & 36.11\% & 35.85\% & 67.38\% & 68.86\% & 68.39\% \\
178 & 35.59\% & 36.11\% & 35.85\% & 67.38\% & 68.86\% & 68.39\% \\
179 & 35.59\% & 36.11\% & 35.85\% & 67.38\% & 68.86\% & 68.39\% \\
180 & 35.59\% & 36.11\% & 35.85\% & 67.38\% & 68.86\% & 68.39\% \\
\hline
\end{tabular}

\end{table}





% \begin{table}[tb]
% \caption{Statistics of the numbers of killed mutants over minutes}
% \label{table:timetable} 
% \footnotesize
% \centering
% \begin{tabular}{c|rrr|rrr}
% % @{\hspace{1pt}}p{9mm}
% % @{\hspace{2pt}}|
% % @{\hspace{1pt}}>{\raggedleft\arraybackslash}p{8mm}@{\hspace{1pt}}|
% % @{\hspace{1pt}}>{\raggedleft\arraybackslash}p{17mm}@{\hspace{1pt}}|
% % @{\hspace{1pt}}>{\raggedleft\arraybackslash}p{28mm}@{\hspace{1pt}}|
% % @{\hspace{1pt}}>{\raggedleft\arraybackslash}p{14mm}@{\hspace{1pt}}|
% % }
% \hline
% \textbf{Time}  & \multicolumn{3}{c|}{\textbf{MLFS}} & \multicolumn{3}{c}{\textbf{LIBU}} \\
% (minute) 
% & \multicolumn{1}{c}{min} & \multicolumn{1}{c}{max} & \multicolumn{1}{c|}{avg.}
% & \multicolumn{1}{c}{min} & \multicolumn{1}{c}{max} & \multicolumn{1}{c}{avg.} \\
% \hline
% 0 & 76 & 76 & 76.0 & 301 & 302 & 301.4 \\ 
% 1 & 867 & 895 & 882.7 & 396 & 404 & 401.4 \\ 
% 2 & 947 & 959 & 953.8 & 401 & 410 & 405.9 \\ 
% 3 & 994 & 1017 & 1005.9 & 401 & 410 & 406.9 \\ 
% 4 & 1029 & 1047 & 1037.7 & 404 & 410 & 407.5 \\ 
% 5 & 1060 & 1081 & 1067.9 & 404 & 412 & 408.1 \\ 
% 6 & 1079 & 1100 & 1088.8 & 404 & 412 & 408.9 \\ 
% 7 & 1092 & 1115 & 1104.7 & 404 & 413 & 410.6 \\ 
% 8 & 1105 & 1134 & 1119.0 & 405 & 414 & 411.4 \\ 
% 9 & 1118 & 1148 & 1131.1 & 407 & 415 & 412.3 \\ 
% 10 & 1132 & 1158 & 1143.1 & 407 & 416 & 412.9 \\ 
% 11 & 1140 & 1171 & 1153.4 & 407 & 417 & 413.3 \\ 
% 12 & 1152 & 1177 & 1162.5 & 408 & 417 & 413.4 \\ 
% 13 & 1159 & 1184 & 1170.7 & 408 & 417 & 413.5 \\ 
% 14 & 1170 & 1188 & 1178.8 & 408 & 417 & 413.5 \\ 
% 15 & 1177 & 1195 & 1185.9 & 408 & 417 & 413.6 \\ 
% 16 & 1184 & 1203 & 1192.7 & 408 & 417 & 413.6 \\ 
% 17 & 1189 & 1208 & 1198.5 & 408 & 417 & 413.8 \\ 
% 18 & 1196 & 1216 & 1203.8 & 408 & 417 & 413.8 \\ 
% 19 & 1199 & 1221 & 1208.3 & 408 & 417 & 413.8 \\ 
% 20 & 1202 & 1228 & 1212.8 & 408 & 417 & 413.8 \\ 
% 21 & 1206 & 1235 & 1218.3 & 408 & 417 & 413.8 \\ 
% 22 & 1209 & 1239 & 1222.8 & 408 & 417 & 414.0 \\ 
% 23 & 1213 & 1243 & 1226.7 & 408 & 417 & 414.1 \\ 
% 24 & 1216 & 1246 & 1230.5 & 409 & 417 & 414.2 \\ 
% 25 & 1219 & 1248 & 1234.1 & 409 & 417 & 414.2 \\ 
% 26 & 1224 & 1252 & 1237.2 & 409 & 417 & 414.2 \\ 
% 27 & 1228 & 1253 & 1239.9 & 409 & 417 & 414.2 \\ 
% 28 & 1232 & 1258 & 1244.1 & 409 & 417 & 414.2 \\ 
% 29 & 1234 & 1258 & 1247.6 & 409 & 417 & 414.2 \\ 
% 30 & 1235 & 1260 & 1249.7 & 409 & 417 & 414.2 \\ 
% 31 & 1239 & 1265 & 1252.9 & 409 & 417 & 414.2 \\ 
% 32 & 1244 & 1268 & 1255.5 & 409 & 417 & 414.2 \\ 
% 33 & 1248 & 1270 & 1258.0 & 409 & 417 & 414.2 \\ 
% 34 & 1252 & 1273 & 1260.4 & 409 & 417 & 414.2 \\ 
% 35 & 1255 & 1275 & 1263.3 & 409 & 417 & 414.2 \\ 
% 36 & 1256 & 1277 & 1266.4 & 409 & 417 & 414.2 \\ 
% 37 & 1256 & 1279 & 1268.7 & 409 & 417 & 414.2 \\ 
% 38 & 1260 & 1282 & 1271.2 & 409 & 417 & 414.3 \\ 
% 39 & 1267 & 1283 & 1273.4 & 409 & 417 & 414.3 \\ 
% 40 & 1268 & 1285 & 1275.8 & 409 & 417 & 414.4 \\ 
% 41 & 1271 & 1286 & 1278.5 & 409 & 417 & 414.4 \\ 
% 42 & 1274 & 1289 & 1281.4 & 409 & 417 & 414.4 \\ 
% 43 & 1275 & 1292 & 1283.6 & 409 & 417 & 414.4 \\ 
% 44 & 1277 & 1293 & 1285.3 & 409 & 417 & 414.4 \\ 
% 45 & 1279 & 1297 & 1287.3 & 409 & 417 & 414.4 \\ 
% 46 & 1284 & 1298 & 1289.2 & 409 & 417 & 414.4 \\ 
% 47 & 1285 & 1299 & 1291.0 & 409 & 417 & 414.5 \\ 
% 48 & 1286 & 1302 & 1292.9 & 409 & 417 & 414.5 \\ 
% 49 & 1287 & 1303 & 1294.6 & 409 & 417 & 414.5 \\ 
% 50 & 1291 & 1303 & 1296.4 & 409 & 417 & 414.5 \\ 
% 51 & 1293 & 1305 & 1298.1 & 409 & 417 & 414.5 \\ 
% 52 & 1294 & 1308 & 1299.7 & 409 & 417 & 414.5 \\ 
% 53 & 1294 & 1309 & 1300.9 & 409 & 417 & 414.5 \\ 
% 54 & 1295 & 1313 & 1302.7 & 409 & 417 & 414.5 \\ 
% 55 & 1295 & 1316 & 1304.4 & 409 & 417 & 414.5 \\ 
% 56 & 1295 & 1318 & 1305.7 & 409 & 417 & 414.6 \\ 
% 57 & 1296 & 1320 & 1307.9 & 409 & 417 & 414.6 \\ 
% 58 & 1301 & 1322 & 1310.0 & 409 & 417 & 414.6 \\ 
% 59 & 1301 & 1325 & 1311.6 & 409 & 417 & 414.6 \\ 
% 60 & 1302 & 1325 & 1312.8 & 409 & 417 & 414.6 \\ 
% 61 & 1303 & 1328 & 1314.3 & 409 & 417 & 414.6 \\ 
% 62 & 1303 & 1328 & 1315.1 & 409 & 417 & 414.6 \\ 
% 63 & 1303 & 1329 & 1316.4 & 409 & 417 & 414.6 \\ 
% 64 & 1304 & 1329 & 1318.1 & 409 & 417 & 414.6 \\ 
% 65 & 1305 & 1330 & 1319.6 & 409 & 417 & 414.6 \\ 
% 66 & 1305 & 1331 & 1320.5 & 409 & 417 & 414.6 \\ 
% 67 & 1307 & 1332 & 1321.9 & 409 & 417 & 414.6 \\ 
% 68 & 1309 & 1334 & 1322.8 & 409 & 417 & 414.6 \\ 
% 69 & 1311 & 1334 & 1324.3 & 409 & 417 & 414.6 \\ 
% 70 & 1314 & 1335 & 1325.7 & 409 & 417 & 414.6 \\ 
% \hline
% \end{tabular}
% \end{table}


% \begin{table}[tb]
% \caption{Statistics of the numbers of killed mutants over minutes 2}
% \label{table:timetable2} 
% \footnotesize
% \centering
% \begin{tabular}{c|rrr|rrr}
% \hline
% \textbf{Time}  & \multicolumn{3}{c|}{\textbf{MLFS}} & \multicolumn{3}{c}{\textbf{LIBU}} \\
% (minute) 
% & \multicolumn{1}{c}{min} & \multicolumn{1}{c}{max} & \multicolumn{1}{c|}{avg.}
% & \multicolumn{1}{c}{min} & \multicolumn{1}{c}{max} & \multicolumn{1}{c}{avg.} \\
% \hline
% 71 & 1316 & 1336 & 1327.4 & 409 & 417 & 414.6 \\ 
% 72 & 1316 & 1339 & 1328.9 & 409 & 417 & 414.6 \\ 
% 73 & 1317 & 1342 & 1330.4 & 409 & 417 & 414.6 \\ 
% 74 & 1318 & 1343 & 1331.9 & 409 & 417 & 414.6 \\ 
% 75 & 1319 & 1345 & 1333.3 & 409 & 417 & 414.6 \\ 
% 76 & 1321 & 1346 & 1334.5 & 409 & 417 & 414.6 \\ 
% 77 & 1322 & 1347 & 1335.9 & 409 & 417 & 414.6 \\ 
% 78 & 1323 & 1348 & 1337.1 & 409 & 417 & 414.6 \\ 
% 79 & 1325 & 1349 & 1338.1 & 409 & 417 & 414.6 \\ 
% 80 & 1325 & 1349 & 1338.8 & 409 & 417 & 414.6 \\ 
% 81 & 1328 & 1351 & 1340.0 & 409 & 417 & 414.6 \\ 
% 82 & 1330 & 1352 & 1341.3 & 409 & 417 & 414.6 \\ 
% 83 & 1331 & 1353 & 1342.2 & 409 & 417 & 414.6 \\ 
% 84 & 1333 & 1353 & 1342.9 & 409 & 417 & 414.6 \\ 
% 85 & 1334 & 1353 & 1343.7 & 409 & 417 & 414.6 \\ 
% 86 & 1335 & 1354 & 1344.3 & 409 & 417 & 414.6 \\ 
% 87 & 1336 & 1355 & 1345.7 & 409 & 417 & 414.6 \\ 
% 88 & 1339 & 1355 & 1346.7 & 409 & 417 & 414.6 \\ 
% 89 & 1340 & 1356 & 1348.5 & 409 & 418 & 414.8 \\ 
% 90 & 1340 & 1356 & 1348.9 & 409 & 418 & 414.8 \\ 
% 91 & 1341 & 1357 & 1350.2 & 409 & 418 & 414.8 \\ 
% 92 & 1341 & 1358 & 1350.7 & 409 & 418 & 414.8 \\ 
% 93 & 1341 & 1359 & 1351.3 & 409 & 418 & 414.8 \\ 
% 94 & 1342 & 1359 & 1351.8 & 409 & 418 & 414.8 \\ 
% 95 & 1342 & 1362 & 1352.4 & 409 & 418 & 414.8 \\ 
% 96 & 1345 & 1362 & 1353.3 & 409 & 418 & 414.8 \\ 
% 97 & 1347 & 1362 & 1354.3 & 409 & 418 & 414.8 \\ 
% 98 & 1348 & 1363 & 1355.3 & 409 & 418 & 414.8 \\ 
% 99 & 1348 & 1364 & 1355.7 & 409 & 418 & 414.8 \\ 
% 100 & 1348 & 1364 & 1356.4 & 409 & 418 & 414.8 \\ 
% 101 & 1349 & 1364 & 1356.7 & 409 & 418 & 414.8 \\ 
% 102 & 1349 & 1364 & 1357.5 & 409 & 418 & 414.8 \\ 
% 103 & 1349 & 1364 & 1358.1 & 409 & 418 & 414.8 \\ 
% 104 & 1351 & 1364 & 1358.7 & 409 & 418 & 414.8 \\ 
% 105 & 1353 & 1365 & 1359.3 & 409 & 418 & 414.8 \\ 
% 106 & 1353 & 1367 & 1360.4 & 409 & 418 & 414.8 \\ 
% 107 & 1353 & 1368 & 1360.9 & 409 & 418 & 414.8 \\ 
% 108 & 1353 & 1369 & 1361.9 & 409 & 418 & 414.8 \\ 
% 109 & 1354 & 1369 & 1362.6 & 409 & 418 & 414.8 \\ 
% 110 & 1354 & 1370 & 1363.2 & 409 & 418 & 414.8 \\ 
% 111 & 1355 & 1370 & 1363.7 & 409 & 418 & 414.8 \\ 
% 112 & 1355 & 1370 & 1364.0 & 409 & 418 & 414.8 \\ 
% 113 & 1359 & 1371 & 1365.1 & 409 & 418 & 414.8 \\ 
% 114 & 1361 & 1371 & 1365.6 & 409 & 418 & 414.8 \\ 
% 115 & 1362 & 1372 & 1366.2 & 409 & 418 & 414.8 \\ 
% 116 & 1362 & 1374 & 1366.8 & 409 & 418 & 414.8 \\ 
% 117 & 1362 & 1374 & 1367.1 & 409 & 418 & 414.8 \\ 
% 118 & 1363 & 1374 & 1367.8 & 409 & 418 & 414.8 \\ 
% 119 & 1364 & 1374 & 1368.7 & 409 & 418 & 414.8 \\ 
% 120 & 1364 & 1374 & 1369.0 & 409 & 418 & 414.8 \\ 
% 121 & 1364 & 1374 & 1369.5 & 409 & 418 & 414.9 \\ 
% 122 & 1364 & 1375 & 1370.4 & 409 & 418 & 415.0 \\ 
% 123 & 1366 & 1376 & 1371.5 & 409 & 418 & 415.0 \\ 
% 124 & 1367 & 1377 & 1372.1 & 409 & 418 & 415.0 \\ 
% 125 & 1367 & 1377 & 1372.6 & 409 & 418 & 415.0 \\ 
% 126 & 1367 & 1377 & 1372.8 & 409 & 418 & 415.0 \\ 
% 127 & 1367 & 1380 & 1373.5 & 409 & 418 & 415.0 \\ 
% 128 & 1369 & 1381 & 1374.3 & 409 & 418 & 415.0 \\ 
% 129 & 1369 & 1382 & 1375.0 & 409 & 418 & 415.0 \\ 
% 130 & 1369 & 1382 & 1375.3 & 409 & 418 & 415.0 \\ 
% 131 & 1369 & 1382 & 1375.9 & 409 & 418 & 415.0 \\ 
% 132 & 1369 & 1383 & 1376.1 & 409 & 418 & 415.0 \\ 
% 133 & 1370 & 1383 & 1376.8 & 409 & 418 & 415.0 \\ 
% 134 & 1371 & 1383 & 1377.0 & 409 & 418 & 415.0 \\ 
% 135 & 1371 & 1383 & 1377.6 & 409 & 418 & 415.0 \\ 
% 136 & 1371 & 1384 & 1378.2 & 409 & 418 & 415.0 \\ 
% 137 & 1371 & 1384 & 1378.4 & 409 & 418 & 415.0 \\ 
% 138 & 1371 & 1387 & 1379.4 & 409 & 418 & 415.0 \\ 
% 139 & 1371 & 1388 & 1379.6 & 409 & 418 & 415.0 \\ 
% 140 & 1372 & 1388 & 1380.1 & 409 & 418 & 415.1 \\ 
% \hline
% \end{tabular}
% \end{table}


% \begin{table}[tb]
% \caption{Statistics of the numbers of killed mutants over minutes 3}
% \label{table:timetable3} 
% \footnotesize
% \centering
% \begin{tabular}{c|rrr|rrr}
% \hline
% \textbf{Time}  & \multicolumn{3}{c|}{\textbf{MLFS}} & \multicolumn{3}{c}{\textbf{LIBU}} \\
% (minute) 
% & \multicolumn{1}{c}{min} & \multicolumn{1}{c}{max} & \multicolumn{1}{c|}{avg.}
% & \multicolumn{1}{c}{min} & \multicolumn{1}{c}{max} & \multicolumn{1}{c}{avg.} \\
% \hline
% 141 & 1374 & 1389 & 1381.2 & 409 & 418 & 415.1 \\ 
% 142 & 1374 & 1389 & 1381.3 & 409 & 418 & 415.1 \\ 
% 143 & 1375 & 1389 & 1382.0 & 409 & 418 & 415.1 \\ 
% 144 & 1375 & 1389 & 1382.5 & 409 & 418 & 415.1 \\ 
% 145 & 1376 & 1390 & 1383.1 & 409 & 418 & 415.1 \\ 
% 146 & 1376 & 1390 & 1383.2 & 409 & 418 & 415.1 \\ 
% 147 & 1376 & 1390 & 1383.4 & 409 & 418 & 415.1 \\ 
% 148 & 1377 & 1390 & 1384.0 & 409 & 418 & 415.1 \\ 
% 149 & 1377 & 1391 & 1384.7 & 409 & 418 & 415.1 \\ 
% 150 & 1377 & 1391 & 1384.9 & 409 & 418 & 415.1 \\ 
% 151 & 1379 & 1392 & 1385.8 & 409 & 418 & 415.1 \\ 
% 152 & 1379 & 1392 & 1386.5 & 409 & 418 & 415.1 \\ 
% 153 & 1380 & 1393 & 1386.7 & 409 & 418 & 415.1 \\ 
% 154 & 1380 & 1393 & 1386.9 & 409 & 418 & 415.1 \\ 
% 155 & 1380 & 1394 & 1387.1 & 409 & 418 & 415.1 \\ 
% 156 & 1380 & 1395 & 1387.8 & 409 & 418 & 415.1 \\ 
% 157 & 1380 & 1395 & 1388.1 & 409 & 418 & 415.1 \\ 
% 158 & 1381 & 1396 & 1388.7 & 409 & 418 & 415.1 \\ 
% 159 & 1381 & 1396 & 1389.1 & 409 & 418 & 415.1 \\ 
% 160 & 1381 & 1398 & 1389.8 & 409 & 418 & 415.1 \\ 
% 161 & 1382 & 1401 & 1390.7 & 409 & 418 & 415.1 \\ 
% 162 & 1383 & 1401 & 1391.4 & 409 & 418 & 415.1 \\ 
% 163 & 1385 & 1402 & 1392.4 & 409 & 418 & 415.1 \\ 
% 164 & 1385 & 1403 & 1393.2 & 409 & 418 & 415.1 \\ 
% 165 & 1385 & 1403 & 1393.6 & 409 & 418 & 415.1 \\ 
% 166 & 1385 & 1404 & 1394.3 & 409 & 418 & 415.1 \\ 
% 167 & 1385 & 1405 & 1395.0 & 409 & 418 & 415.1 \\ 
% 168 & 1385 & 1405 & 1395.0 & 409 & 418 & 415.1 \\ 
% 169 & 1385 & 1405 & 1395.0 & 409 & 418 & 415.1 \\ 
% 170 & 1385 & 1405 & 1395.0 & 409 & 418 & 415.1 \\ 
% 171 & 1385 & 1405 & 1395.0 & 409 & 418 & 415.1 \\ 
% 172 & 1385 & 1405 & 1395.0 & 409 & 418 & 415.1 \\ 
% 173 & 1385 & 1405 & 1395.0 & 409 & 418 & 415.1 \\ 
% 174 & 1385 & 1405 & 1395.0 & 409 & 418 & 415.1 \\ 
% 175 & 1385 & 1405 & 1395.0 & 409 & 418 & 415.1 \\ 
% 176 & 1385 & 1405 & 1395.0 & 409 & 418 & 415.1 \\ 
% 177 & 1385 & 1405 & 1395.0 & 409 & 418 & 415.1 \\ 
% 178 & 1385 & 1405 & 1395.0 & 409 & 418 & 415.1 \\ 
% 179 & 1385 & 1405 & 1395.0 & 409 & 418 & 415.1 \\ 
% 180 & 1385 & 1405 & 1395.0 & 409 & 418 & 415.1 \\
% \hline
% \end{tabular}

% \end{table}


